Tropical Lagrangians in toric del-Pezzo surfaces

We look at how one can construct from the data of a dimer model a Lagrangian submanifold in $(\mathbb{C}^*)^n$ whose valuation projection approximates a tropical hypersurface. Each face of the dimer corresponds to a Lagrangian disk with boundary on our tropical Lagrangian submanifold, forming a Lagrangian mutation seed. Using this we find tropical Lagrangian tori $L_{T^2}$ in the complement of a smooth anticanonical divisor of a toric del-Pezzo whose wall-crossing transformations match those of monotone SYZ fibers. An example is worked out for the mirror pair $(\mathbb{CP}^2\setminus E, W), \check X_{9111}$. We find a symplectomorphism of $\mathbb{CP}^2\setminus E$ interchanging $L_{T^2}$ and a SYZ fiber. Evidence is provided that this symplectomorphism is mirror to fiberwise Fourier-Mukai transform on $\check X_{9111}$.

==> amodelcp2.tex <==

\subsection{\texorpdfstring{$B$}{B}-Model on Projective.}
The story that we want to tell comes from the fibration $\check X_{9111}\to \CP^2$, and understanding how the fibration given by $\check W$ relates to that fibration.
The model which is slightly easier to explore (as homological mirror symmetry has been proven for this pair) is to explore $\Fuk (\check X, \check W)$.
\begin{claim}
	Let $L(k)$ be the mirror to $\mathcal O(k)$. The number of intersection points between $L(k)$ and $L(0)$ is $\frac{k-1}{k-2}{2}$.
\end{claim}
\begin{proof}
	Wrapping the Lagrangian adds a Dehn twist in, so that $\#(L(k)\cap L(0))= \#(L(k-1)\cap L(0))+9$. This allows us to break into the following three cases:
	\begin{itemize}
		\item
		      If $k\cong 0 \mod 3$, then
		      \[
				  \#(L(k)\cap L(0))= 1+ \sum_{i=1}^{k/3} 9i=\frac{(k-1)(k-2)}{2}.
			\]
		\item
		      If $k\cong 1\mod 3$, then
		      \[
			      \#(L(k)\cap L(0))=  \sum_{i=1}^{(k-1)/3} 3+9i= \frac{(k-1)(k-2)}{2}.
		      \]
		\item
		      If $k\cong 2\mod 3$, then
		      \[
			      \#(L(k)\cap L(0))=  \sum_{i=1}^{(k-2)/3} 3+9i= \frac{(k-1)(k-2)}{2}.
		      \]
	\end{itemize}
\end{proof}
From this, we get a tropical genus degree formula for tropical curves.
\begin{corollary}
	Let $\phi$ be an admissible tropical polynomial of degree $d$. Then $g(L(\phi)=\frac{(k-1)(k-2)}{2}$.
\end{corollary}
The genus governs how we can mutate each of these Lagrangians. As an example, let $\phi$ be define an elliptic tropical Lagrangian $L(\phi)$. As a collection of thimbles, the Lagrangian $L(\phi)$ can be mutated along the thimble representing the zero section (See \cref{fig:ellipticmutation}>) It is still unclear what this mutation means in terms of wall-crossing on the moduli space of elliptic tropical Lagrangians, or if there are other such mutations.
\begin{figure}
	\caption{Mutation of the tropical elliptic}
	\label{fig:ellipticmutation}
\end{figure}
By using Claim \cref{claim:surgeryatinfty}, we can take any of the Lagrangians $L(\phi)$ and draw them as Lagrangian gloves. These gloves are constructed by first taking the standard thimble representation of $L(\phi)$, and then at each crossing resolving the intersection of thimbles as a glove. In \cref{fig:gloveforelliptic}, it is clearly seen that Lagrangian $L(\phi)$ for $\phi$ a degree 4 polynomial $\phi$ has the proper genus.
\begin{figure}
	\centering
	\input{figures/gloveforelliptic.tikz}
	\caption{A Lagrangian glove for $L(\phi)$, where $\phi$ is a homogeneous degree 4 polynomial. This is two Lagrangian thimbles, whose intersection point has been resolved as a Lagrangian cobordism.}
	\label{fig:gloveforelliptic}
\end{figure}
The admissible tropical polynomials for $(X^\vee, W^\vee)$ are exactly the homogeneous polynomials, and their tropical Lagrangians are mirror to the corresponding divisor of the polynomial on $X$. In this setting, there is not a lot more to work out.

\subsection{\texorpdfstring{$A$}{A}-Model on \texorpdfstring{$X$}{X}}
This setting has not been explored in much detail. We first understand $X$ via a Lefschetz fibration of $X$. Associated to $E\subset \CP^2$, we have a \emph{Hesse Pencil} of elliptics. By blowing up $\CP^2$ along the base points of the pencil, we arrive get an elliptic surface $X_{3333}$ (using notation from \cite{Miranda1986}). \\
This elliptic pencil  gives us a Lefschetz fibration $W:\CP^2\setminus E \to \CP^1$, with 4 nodal fibers of type $I_3$. Each fiber of this fibration is an elliptic curve missing 9 points. In the standard form, $W:X\to \CC$ has 3 nodal fibers at cubic roots of unity, and at 0. \\
The 12 vanishing cycles of this sit in the homology classes  $\langle 1, 0\rangle , \langle 0, 1 \rangle, \langle -1, 1\rangle$ and $\langle 1, 1\rangle$, as drawn in \cref{fig:x3333}.
\begin{figure}
	\centering
	\input{figures/x3333.tikz}
	\caption{The vanishing cycles of the fibration $X_{3333}$}
	\label{fig:x3333}
\end{figure}

Let $\ell_0$ be a vanishing cycle in the class of $\langle 0, 1\rangle$ , and let $\gamma$ be a small loop around the point $p$. Since the monodromy around $p$ is trivial, we can build a Lagrangian torus $F$ by taking the parallel transport of $\ell_1$ around $\gamma$, which we will think of as a fiber of the moment map. \\
We can alternatively let $\ell_1$ be a vanishing cycle in the class $\langle 1, 0\rangle$, and parallel transport that around $\gamma$. The resulting Lagrangian $L$ will give us a different Lagrangian, which we will think of as the tropical Lagrangian torus as drawn in ...
As we increase the size of $\gamma$ so that it passes $0$, we get a degeneration of both of these Lagrangians. The Lagrangian $F'$ undergoes wall crossing, while the Lagrangian torus is turned into a glove with 3 fingers. \\
